No More Ambiguity in 360{\deg} Room Layout via Bi-Layout Estimation

Inherent ambiguity in layout annotations poses significant challenges to developing accurate 360{\deg} room layout estimation models. To address this issue, we propose a novel Bi-Layout model capable of predicting two distinct layout types. One stops at ambiguous regions, while the other extends to encompass all visible areas. Our model employs two global context embeddings, where each embedding is designed to capture specific contextual information for each layout type. With our novel feature guidance module, the image feature retrieves relevant context from these embeddings, generating layout-aware features for precise bi-layout predictions. A unique property of our Bi-Layout model is its ability to inherently detect ambiguous regions by comparing the two predictions. To circumvent the need for manual correction of ambiguous annotations during testing, we also introduce a new metric for disambiguating ground truth layouts. Our method demonstrates superior performance on benchmark datasets, notably outperforming leading approaches. Specifically, on the MatterportLayout dataset, it improves 3DIoU from 81.70% to 82.57% across the full test set and notably from 54.80% to 59.97% in subsets with significant ambiguity. Project page: https://liagm.github.io/Bi_Layout/

==> figs/ambiguity.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/src/ambiguity_relabel.pdf}
    \caption{\textbf{Ambiguity in Dataset Labels.}\todo{need to re-draw GT with consistent color, and add BEV view}}
    \label{fig:ambiguity}
\end{figure}


==> figs/relabel.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/src/relabel.pdf}
    \caption{\textbf{Relabel Example.}}
    \label{fig:relabel}
\end{figure}


==> figs/teaser.tex <==
% Use figure* for multi-column figure
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth]{figs/src/teaser.pdf}
    \caption{\textbf{Our teaser.}}
    \label{fig:teaser}
\end{figure*}


==> latexmkrc <==
$pdflatex = 'pdflatex %O %S; ps2pdf14 -dPDFSETTINGS=/prepress %B.pdf %B-embed.pdf; mv %B-embed.pdf %B.pdf';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/fullset.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
\vspace{-4mm}
\centering
  \resizebox{0.95\linewidth}{!} % or it will overfull
  {
    \centering
    \begin{tabular}{lccccccc}
    \toprule
        Full set& & \multicolumn{2}{c}{MatterportLayout~\cite{zou2021manhattan}} & \multicolumn{2}{c}{ZInD-Simple~\cite{cruz2021zillow}} & \multicolumn{2}{c}{ZInD-All~\cite{cruz2021zillow}} \\
    \midrule
    Method & \# Params & 2DIoU(\%) & 3DIoU(\%) & 2DIoU(\%) & 3DIoU(\%) & 2DIoU(\%) & 3DIoU(\%) \\
    \midrule
    LED${^2}$Net~\cite{wang2021led2} & {82 M} & 82.37 & 80.05 & 90.20 & 88.34 & 82.31 & 80.28 \\
    LGT-Net~\cite{jiang2022lgt} & 136 M & 83.52 & 81.11 & 91.77 & 89.95 & 84.07 & 82.09 \\
    DOP-Net~\cite{shen2023dopnet} & 137 M & 84.11 & 81.70  & 91.94 & 90.13 & 83.92 & 81.87 \\
    % Ours 512 (original) & 102 M & 84.11 & 81.64 & 91.98 & 90.21 & - & - \\
    Ours (equivalent branch) & {102 M} & \blue{84.56} & \blue{82.05} & \blue{92.07} & \blue{90.25} & \blue{84.90} & \blue{82.96} \\
    % Ours (tolerance) & 102 M & 84.50 & 82.01 & 92.77 & 90.98 & - & - \\
    \midrule
    Ours (disambiguate) & {102 M} & \red{85.10} & \red{82.57} & \red{92.79} & \red{90.95} & \red{86.21} & \red{84.22} \\
    \bottomrule
    \end{tabular}%
  }
  \vspace{-2mm}
  \caption{\textbf{Fullset evaluation.} \red{Red} and \blue{blue} indicate the best and second-best, respectively. \textbf{Equivalent branch} represents the output which is trained with the same label as baseline methods. \textbf{Disambiguate} is our proposed metric.}
  \vspace{-6mm}
  \label{tab:fullset}%
\end{table*}%


==> tables/matterport.tex <==
\begin{table}
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method&2DIoU(\%) &3DIoU(\%) \\
\midrule
HorizonNet~\cite{sun2019horizonnet} & 81.71 & 79.11	 \\
LE$\mathrm{D}^{2}$-Net~\cite{wang2021led2} & 82.61 & 80.14 \\
LGT-Net~\cite{jiang2022lgt} & 83.52 & 81.11	 \\
DOP-Net~\cite{shen2023dopnet} & 84.11 & 81.70	 \\
Our original branch & \textbf{84.40} & \textbf{81.96} \\
Our oracle & \textbf{85.25} & \textbf{82.76} \\
\bottomrule
\end{tabular}
}
\caption{Quantitative results of general layout estimation evaluated on MatterportLayout~\cite{zou2021manhattan} dataset.
}
\label{tab:matterport}
\vspace{-2mm}
\end{table}

==> tables/opening.tex <==
\begin{table}
  \centering
    \begin{tabular}{lcc}
    \toprule
    Dataset & Precision & Recall \\
    \midrule
    %MatterportLayout~\cite{zou2021manhattan} & 0.708 \\
    ZInD-All~\cite{cruz2021zillow} & 0.82 & 0.71 \\
    \bottomrule
    \end{tabular}%
  \caption{\textbf{Ambiguity detection} on ZInD~\cite{cruz2021zillow} dataset.}
  \vspace{-7mm}
  \label{tab:opening}%
\end{table}%

==> tables/subset.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}
\centering
\vspace{-4mm}
  \resizebox{0.95\linewidth}{!} % or it will overfull
  {
  \centering
    \begin{tabular}{lccccccc}
    \toprule
          Subset& & \multicolumn{2}{c}{MatterportLayout~\cite{zou2021manhattan}} & \multicolumn{2}{c}{ZInD-Simple~\cite{cruz2021zillow}} & \multicolumn{2}{c}{ZInD-All~\cite{cruz2021zillow}} \\
    \midrule
    Method & \# Params & 2DIoU(\%) & 3DIoU(\%) & 2DIoU(\%) & 3DIoU(\%) & 2DIoU(\%) & 3DIoU(\%) \\
    \midrule
    LED${^2}$Net~\cite{wang2021led2} & 82 M & 53.57  & 51.12  & 45.31 & 44.10  & 48.76 & 47.35 \\
    LGT-Net~\cite{jiang2022lgt} & 136 M & 53.17 & 50.54 & 53.20 & 52.00 &  50.89 & 49.58 \\
    DOP-Net~\cite{shen2023dopnet} & 137 M & 57.13 & 54.80 & 51.55 & 50.26 &  50.92  &  49.46 \\
    Ours (equivalent branch) & 102 M & \blue{59.85} & \blue{57.08} & \blue{55.09} & \blue{53.76} & \blue{54.22}  & \blue{52.78} \\
    \midrule
    Ours (disambiguate) & 102 M & \red{62.81} & \red{59.97} & \red{62.10} & \red{60.63} & \red{60.20}  & \red{58.53} \\
    \bottomrule
    \end{tabular}%
  }
  \vspace{-2mm}
  \caption{\textbf{Subset evaluation.} \red{Red} and \blue{blue} indicate the best and second-best, respectively. \textbf{Equivalent branch} represents the output which is trained with the same label as baseline methods. \textbf{Disambiguate} is our proposed metric.}
  \vspace{-4mm}
  \label{tab:subset}%
\end{table*}%
